Multinoulli Extension: A Lossless Continuous Relaxation for Partition-Constrained Subset Selection

Identifying the most representative subset for a close-to-submodular objective while satisfying the predefined partition constraint is a fundamental task with numerous applications in machine learning. However, the existing distorted local-search methods are often hindered by their prohibitive query complexities and the rigid requirement for prior knowledge of difficult-to-obtain structural parameters. To overcome these limitations, we introduce a novel algorithm titled Multinoulli-SCG, which not only is parameter-free, but also can achieve the same approximation guarantees as the distorted local-search methods with significantly fewer function evaluations. More specifically, when the objective function is monotone $\alpha$-weakly DR-submodular or $(\gamma,\beta)$-weakly submodular, our Multinoulli-SCG algorithm can attain a value of $(1-e^{-\alpha})\text{OPT}-\epsilon$ or $(\frac{\gamma^{2}(1-e^{-(\beta(1-\gamma)+\gamma^2)})}{\beta(1-\gamma)+\gamma^2})\text{OPT}-\epsilon$ with only $O(1/\epsilon^{2})$ function evaluations, where OPT denotes the optimal value. The cornerstone of our Multinoulli-SCG algorithm is an innovative continuous-relaxation framework named Multinoulli Extension(ME), which can effectively convert the discrete subset selection problem subject to partition constraints into a solvable continuous maximization focused on learning the optimal multinoulli priors across the concerned partition. In sharp contrast with the well-established multi-linear extension for submodular subset selection, a notable advantage of our proposed ME is its intrinsic capacity to provide a lossless rounding scheme for any set function. Furthermore, based on our proposed ME, we also present two novel online algorithms, namely, Multinoulli-OSCG and Multinoulli-OSGA, for the unexplored online subset selection problems over partition constraints.

==> Algorithms.tex <==
In this section, we  delve into the development of efficient approximation algorithms for the subset selection problem~\eqref{equ_problem} based on our  introduced Multinoulli Extension. 
% Regrettably, we observe that, in the worst-case scenario, the stationary points of our proposed Multinoulli Extension only can guarantee a sub-optimal approximation to the maximum value of the subset selection problem~\eqref{equ_problem}. 
%The success of this strategy largely depends on the quality of  the stationary points of our proposed Multinoulli Extension relative to the maximum value of the subset selection problem~\eqref{equ_problem}. 
\subsection{Stochastic Gradient Ascent Algorithm}
In general, a straightforward strategy is to initially apply the well-established Gradient Ascent(GA) method~\citep{nesterov2013introductory,bertsekas2015convex,lan2020first}, to maximize our proposed Multinoulli Extension $F$, and subsequently, to finalize our selection by rounding the resulting continuous solution. However, the implementation of GA often requires accurately computing the gradients of  $F$, which is typically computationally intensive. Fortunately, the first point of Theorem~\ref{thm1} indicates that it is feasible  to sample a sequence of random elements to construct an unbiased estimator for each $\frac{\partial F}{\partial p_{k}^{m}}$. Specifically, when each $e_{\hat{k}}^{\hat{b}}(l)$ is independently drawn from the multinoulli distribution Multi($\p_{\hat{k}}$) for any $\hat{k}\in[K]$, $\hat{b}\in[n_{\hat{k}}] $ and $l\in[L]$, we can estimate $\frac{\partial F}{\partial p_{k}^{m}}(\p_{1},\dots,\p_{K})$ as:
\begin{equation}\label{equ_estimate_gradient}
	\widehat{\frac{\partial F}{\partial p_{k}^{m}}}:=\frac{B_{k}}{L}\sum_{l=1}^{L}\Big(f\Big(v_{k}^{m}\Big|\cup_{\hat{k}=1}^{K}\cup_{\hat{b}=1}^{B_{k}}\{e_{\hat{k}}^{\hat{b}}(l)\}-e_{k}^{1}(l)\Big)\Big).
\end{equation}

By integrating this stochastic gradient into the GA method, we can derive a stochastic variant of gradient ascent method for our proposed Multinoulli Extension, as detailed in Algorithm~\ref{alg_SGA_multi}. 
\begin{algorithm}[t]
	% \small
	\caption{Stochastic Gradient Ascent for Mutinoulli Extension(\textbf{Multinoulli-SGA})}\label{alg_SGA_multi}
	{\bf Input:} Batch size $L$, step size $\eta$, number of iterations $T$, partition $\{\V_{1},\dots,\V_{K}\}$ of set $\V$ where $\V_{k}=\{v_{k}^{1},\dots,v_{k}^{n_{k}}\}$ and the set function $f$
	\begin{algorithmic}[1]
		% \STATE Set $\triangle_{t}=1$ when $t<T$ and $\triangle_{T}=1+\ln(\tau)$ where $\tau=\max(\frac{1}{\gamma},\frac{r^{2}(\mathcal{X})L}{c})$.
		% \STATE Set $\triangle=\sum_{t=1}^{T}\triangle_{t}$
		\STATE \textbf{Initialize} $\x(1)=\left(\p_{1}(1),\dots,\p_{K}(1)\right)\in\prod_{k=1}^{K}\triangle_{n_{k}}$;
		\FOR{$t=1,\dots,T$}
		\STATE  Generate a subset $S_{t}$ by rounding $\x(t)$;
		\STATE Compute  $\widetilde{\nabla}F(\x(t))$ based on Eq.\eqref{equ_estimate_gradient};
		\STATE Set $\y(t+1):=\x(t)+\eta\widetilde{\nabla}F(\x(t))$;
		\STATE $\x(t+1):=\mathop{\arg\min}_{\z\in\prod_{k=1}^{K}\triangle_{n_{k}}}\|\z-\y(t+1)\|_{2}$;
		\ENDFOR
		\STATE Return $S:=\mathop{\arg\max}_{t\in[T]}f(S_{t})$;
	\end{algorithmic}
\end{algorithm}
Furthermore, based on the previous results of Theorem~\ref{thm1} and Theorem~\ref{thm2}, we also can verify that:
\begin{theorem}[Proof provided in \cref{append:proof3}]\label{thm3}When the set function $f:2^{\V}\rightarrow\R_{+}$ is monotone and $\alpha$-weakly DR-submodular, if we set $\eta=\mathcal{O}(\frac{1}{\sqrt{T}})$ and the batch size $L=\mathcal{O}(1)$, the subset $S$ output by Algorithm~\ref{alg_SGA_multi} satisfies:
	\begin{equation*}
		\E\big(f(S)\big)\ge\Big(\frac{\alpha}{1+\alpha}\Big)f(S^{*})-\mathcal{O}(\frac{1}{\sqrt{T}}),
		\end{equation*} where $S^{*}$ is the optimal solution of problem~\eqref{equ_problem}. Similarly, if the set function $f:2^{\V}\rightarrow\R_{+}$ is $(\gamma,\beta)$-weakly monotone submodular, $\eta=\mathcal{O}(\frac{1}{\sqrt{T}})$ and $L=\mathcal{O}(1)$, the returned  subset $S$ of Algorithm~\ref{alg_SGA_multi} satisfies:
	\begin{equation*}
		\E\big(f(S)\big)\ge\Big(\frac{\gamma^{2}}{1+\beta(1-\gamma)+\gamma^{2}}\Big)f(S^{*})-\mathcal{O}(\frac{1}{\sqrt{T}}).
		\end{equation*} 
\end{theorem}
\begin{remark}
Theorem~\ref{thm3} shows that, if the set function $f$  is monotone and $\alpha$-weakly DR-submodular,  after $\mathcal{O}(1/\epsilon^{2})$ iterations, the subset output by our proposed Algorithm~\ref{thm1} can attain $(\frac{\alpha}{1+\alpha})OPT-\epsilon$ where $OPT$ is the  maximum value of problem~\eqref{equ_problem}. Moreover, when $f$ is $(\gamma,\beta)$-weakly monotone  submodular, after $\mathcal{O}(\frac{1}{\epsilon^{2}})$ iterations, Algorithm~\ref{thm1} also can achieve $\Big(\frac{\gamma^{2}}{1+\beta(1-\gamma)+\gamma^{2}}\Big)OPT-\epsilon$.
\end{remark}
In comparison with the state-of-the-art local search methods~\citep{thiery2022two,JOGO-Lu}, our proposed Algorithm~\ref{alg_SGA_multi} is more practical because it does not require prior knowledge of the diminishing-return ratio and submodularity ratios. However, when the set function $f$ is $\alpha$-weakly DR-submodular, the  worst-case $(\frac{\alpha}{1+\alpha})$-approximation of Algorithm~\ref{alg_SGA_multi} is less competitive than the optimal $(1-e^{-\alpha})$-approximation~\citep{harshaw2019submodular}. Furthermore, for $(\gamma,\beta)$-weakly submodular objectives, the  $(\frac{\gamma^{2}}{1+\beta(1-\gamma)+\gamma^{2}})$-approximation provided by Algorithm~\ref{alg_SGA_multi}  is also weaker than the $\frac{\gamma^{2}(1-e^{-(\beta(1-\gamma)+\gamma^2)})}{\beta(1-\gamma)+\gamma^{2}}$-approximation of  ~\citep{thiery2022two}. To circumvent this obstacle, we next present a variant of  Frank-Wolfe method~\citep{lacoste2016convergence,braun2022conditional} to maximize our proposed Multinoulli Extension.


%it is known that  the optimal approximation ratio for $\alpha$-weakly DR-submodular functions is $(1-e^{-\alpha})$~\citep{harshaw2019submodular}. Furthermore, for $(\gamma,\beta)$-weakly submodular objectives, the  $(\frac{\gamma^{2}}{1+\beta(1-\gamma)+\gamma^{2}})$-approximation of Algorithm~\ref{alg_SGA_multi}  is also weaker than the known $\frac{\gamma^{2}(1-e^{-(\beta(1-\gamma)+\gamma^2)})}{\beta(1-\gamma)+\gamma^{2}}$-approximation~ \citep{thiery2022two}. %To match these state-of-the-art approximation guarantees, we next propose a variant of the classical Frank Wolfe method to maximize our proposed Multinoulli Extension.









 
%Nevertheless, it is known that the optimal approximation ratio for $\alpha$-weakly DR-submodular functions is $(1-e^{-\alpha})$~\citep{harshaw2019submodular}. Furthermore, for $(\gamma,\beta)$-weakly submodular objectives, the  $(\frac{\gamma^{2}}{1+\beta(1-\gamma)+\gamma^{2}})$-approximation demonstrated by  Algorithm~\ref{alg_SGA_multi}  is also weaker than the state-of-the-art $\frac{\gamma^{2}(1-e^{-(\beta(1-\gamma)+\gamma^2)})}{\beta(1-\gamma)+\gamma^{2}}$-approximation~ \citep{thiery2022two}. To match these state-of-the-art approximation guarantees, we next propose a variant of the classical Frank Wolfe method to maximize our proposed Multinoulli Extension.






% Recently, a large body of research has demonstrated that, under mild conditions, many first-order gradient algorithms will  converge to a stationary point of the corresponding objective functions~\citep{ghadimi2013stochastic,lacoste2016convergence,allen2018make,drori2020complexity,lan2020first}. Inspired by these findings,  we proceed to
%investigate the stationary points of our proposed Multinoulli Extension. Before going into the details,  we first present the definition of stationary points, that is to say, 
%\begin{definition} Given a differentiable  objective function $G:\mathcal{K}\rightarrow\R$ and a domain $\C\subseteq\mathcal{K}$, a point $\x\in\C$ is called as a stationary point for the function $G$ over the domain $\C$ if and only if $\max_{\y\in\C}\langle\y-\x,\nabla G(\x)\rangle\le 0$.
%\end{definition}
% Next, we detail the specific performance of the stationary points of the Multinoulli Extension relative to the maximum value of problem~\eqref{equ_problem}. Specifically, we have that
%\begin{theorem}[Proof provided in \cref{append:proof3}]\label{thm3} If the set function $f:2^{\V}\rightarrow\R_{+}$ is monotone and $\alpha$-weakly DR-submodular, then for any stationary point $(\p_{1},\dots,\p_{K})$ of its Multinoulli Extension $F$ over the domain $\prod_{k=1}^{K}\Delta_{n_{k}}$, the following inequality holds:
%	\begin{equation*}
	%	F(\p_{1},\dots,\p_{K})\ge\Big(\frac{1}{1+\alpha}\Big)f(S^{*}),
%	\end{equation*} where $S^{*}$ is the optimal solution of problem~\eqref{equ_problem}. Similarly, when the set function $f:2^{\V}\rightarrow\R_{+}$ is monotone and $(\gamma,\beta)$-weakly submodular, for any stationary point $(\p_{1},\dots,\p_{K})$ over the domain $\prod_{k=1}^{K}\Delta_{n_{k}}$ , we also can show that
	%	\begin{equation*}
	%	F(\p_{1},\dots,\p_{K})\ge\Big(\frac{\gamma^{2}}{1+\beta(1-\gamma)+\gamma^{2}}\Big)f(S^{*}).
%	\end{equation*} 
%\end{theorem}%\begin{remark}
%Theorem~\ref{thm3} indicates that when the set function $f$  is monotone and $\alpha$-weakly DR-submodular,  the direct application of standard gradient methods, e.g. Frank Wolfe and gradient ascent, into the relaxed problem~\eqref{equ_prob_relaxed} can guarantee a $(\frac{1}{1+\alpha})$-approximation to the  maximum value of problem~\eqref{equ_problem}. 
%Moreover, when $f$ is monotone and $(\gamma,\beta)$-weakly submodular, Theorem~\ref{thm3} also shows that the stationary point of our proposed  Multinoulli Extension can offer a $(\frac{\gamma^{2}}{1+\beta(1-\gamma)+\gamma^{2}})$-approximation to  the maximum value of problem~\eqref{equ_problem}.
%\end{remark} 
%However, it is known that the optimal approximation ratio for $\alpha$-weakly DR-submodular functions is $(1-e^{-\alpha})$~\citep{harshaw2019submodular}. Furthermore, for $(\gamma,\beta)$-weakly submodular objectives, the $(\frac{\gamma^{2}}{1+\beta(1-\gamma)+\gamma^{2}})$-approximation  is also weaker than the well-established $\frac{\gamma^{2}(1-e^{-(\beta(1-\gamma)+\gamma^2)})}{\beta(1-\gamma)+\gamma^{2}}$-approximation~ \citep{thiery2022two}. To match these state-of-the-art approximation guarantees, we next propose a variant of the classical Frank Wolfe method to maximize our proposed Multinoulli Extension.
\subsection{Stochastic Continuous Greedy Algorithm}
%which means that, for a sufficiently large $T$, $G\big(\x(t+1)\big)-G\big(\x(t)\big)\approx\frac{1}{T}\left\langle\v(t),\nabla G\big(\x(t)\big)\right\rangle\ge \frac{1}{T}\Big(G\big(\x^{*}\big)-G\big(\x(t)\big)\Big)$ such that $(1-\frac{1}{T})\Big(G\big(\x^{*}\big)-G\big(\x(t)\big)\Big)\gtrsim\Big(G\big(\x^{*}\big)-G\big(\x(t+1)\big)\Big)$, where $\x^{*}$ denotes the optimal solution. Therefore, as the CG algorithm iterates, the gap relative to the maximum value $G(\x^{*})$ will progressively reduce. Note that, in Theorem~\ref{thm2}, we establish a similar relationship between our proposed Multinoulli Extension $F$ and the original $f$, which motivates our adoption of the framework of CG algorithm to address the relaxed problem~\eqref{equ_prob_relaxed}.
In this subsection, we aim to present an effective Frank-Wolfe method for maximizing our introduced Multinoulli Extension, which is primarily inspired by the \emph{continuous greedy}(CG) algorithm for the multi-linear extension~\citep{calinescu2011maximizing,bian2017guaranteed,mokhtari2018conditional}.

The CG algorithm typically comprises two key steps: First, it begins with $\x(0)=\textbf{0}$ and then, at each iteration $t\in[T]$,  the algorithm identifies the optimal ascent direction  $\v(t)=\mathop{\arg\max}_{\v\in\C}\left\langle\v,\nabla G\big(\x(t)\big)\right\rangle$ to update the current variable $\x(t)$ according to the rule $\x(t+1)=\x(t)+\frac{1}{T}\v(t)$ where $G$ is the multi-linear extension of a set function $f$ and $\C$ is a convex domain. The motivation behind the CG algorithm is that when $f$ is \emph{submodular}, the inequality $\left\langle\y,\nabla G\big(\x\big)\right\rangle\ge G(\y)-G(\x)$ holds for any feasible $\x,\y$. Note that, in Theorem~\ref{thm2}, we establish a similar relationship between our proposed Multinoulli Extension $F$ and the original set function $f$, which motivates our adoption of the framework of CG algorithm to address the relaxed problem~\eqref{equ_prob_relaxed}.
\begin{algorithm}[t]
	\caption{Stochastic Continuous Greedy Algorithm for Multinoulli Extension(\textbf{Multinoulli-SCG})}\label{alg:scg_mutli}
	{\bf Input:} Batch size $L$, number of iterations $T$, the set function $f$ and partition $\{\V_{1},\dots,\V_{K}\}$ of set $\V$
	\begin{algorithmic}[1]
		\STATE {\bf Initialize:} $\x(0)=\left(\p_{1}(0),\dots,\p_{K}(0)\right)=\textbf{0}$;
		\FOR{$t=1,\dots,T$}
		\IF[Gradient Estimation(Lines 3-13)]{$t=1$}
		\STATE Compute $\frac{\partial F}{\partial p_{k}^{m}}(\textbf{0})=f(v_{k}^{m}), \forall m\in[n_{k}], k\in[K]$;
		\STATE Set $\boldsymbol{\mathrm{d}}(0)=\nabla F(\textbf{0})$;	
		\ELSE[Differential Estimator(Lines 7-11)] 
		\STATE Sample $\{a(1),\dots,a(L)\}$ uniformly from $[0,1]$;
		\STATE Set $\x_{l}(t)=a(l)\x(t)+(1-a(l))\x(t-1),\forall l\in[L]$; 
		\STATE Compute the Hessian estimator $\widetilde{\nabla}^{2} F\big(\x_{l}(t)\big)$ based on Remark~\ref{remark:estimate_2_order} and Theorem~\ref{thm4} for any $l\in[L]$;
		\STATE Compute $\widetilde{\nabla}^{2}_{t}:=\frac{1}{L}\sum_{l=1}^{L} \widetilde{\nabla}^{2}F\big(\x_{l}(t)\big)$;
		\STATE Compute  $\boldsymbol{\xi}_{t}:=\widetilde{\nabla}^{2}_{t}\big(\x(t)-\x(t-1)\big)$;
		\STATE Aggregate the estimator $\boldsymbol{\mathrm{d}}(t)=\boldsymbol{\mathrm{d}}(t-1)+\boldsymbol{\xi}_{t}$;
		\ENDIF\COMMENT{Stochastic Gradient Ascent(Lines14-15)}
		\STATE Find $\v(t)=\mathop{\arg\max}_{\v\in\prod_{k=1}^{K}\Delta_{n_{k}}}\left\langle\v,\boldsymbol{\mathrm{d}}(t)\right\rangle$;
		\STATE Update $\x(t+1)=\x(t)+\frac{1}{T}\v(t)$ where we set  $\x(t+1):=\big(\p_{1}(t+1),\dots,\p_{K}(t+1)\big)$;
		\ENDFOR
		%\STATE Set $S=\emptyset$;
		%\FOR{$k=1,\dots,K$}
		%	\WHILE{$|S\cap\V_{k}|\le B_{k}$}
		% \STATE Generate a element $e$ from $\V_{k}\cup\{\emptyset\}$ according to the multinoulli distribution Multi($\p_{k}(T)$);
		%  \STATE $S=S\cup\{e\}$;
		%	\ENDWHILE
		%	\ENDFOR
		\STATE  Return $S$ by rounding $\x(T)$;
	\end{algorithmic}
\end{algorithm}	
%we also adopt the stochastic approximation.同样地,为了避免确切的计算Multinoulli Extension的gradient and 有效地 reduce the sample complexity of CG algorithm as much as possible,

Similarly, to avoid the precise computation of the gradients of our proposed Multinoulli Extension, we utilize the stochastic gradients. Additionally, to further reduce the sample complexity, we incorporate the stochastic path-integrated differential estimator~\citep{fang2018spider,yurtsever2019conditional,hassani2020stochastic}, namely, for a sequence of iterations $\{\x(t)\}_{t=0}^{T}$, we estimate each gradient $\nabla F\big(\x(t)\big)$ by the following path-integral form: $\widetilde{\nabla}F\big(\x(t)\big):=\nabla F\big(\x(0)\big)+\sum_{s=1}^{t}\boldsymbol{\xi}_{s}$,
where each $\boldsymbol{\xi}_{s}$ is an unbiased estimator for the difference $\textbf{Diff}_{s}:=\nabla F(\x(s))-\nabla F(\x(s-1))$. Note that, for any $s\in[T]$, the difference $\textbf{Diff}_{s}$ can be rewritten as: $\textbf{Diff}_{s}=\int_{0}^{1}\nabla^{2}F(\x^{a}(s))\mathrm{d}a\Big(\x(s)-\x(s-1)\Big)$, where  $\x^{a}(s)=a\x(s)+(1-a)\x(s-1),\forall a\in[0,1]$ and $\nabla^{2}F$ is the Hessian of $F$. Hence, if we uniformly sample the parameter $a$ from $[0,1]$, the difference $\textbf{Diff}_{s}$ can be unbiasedly estimated by $\boldsymbol{\xi}_{s}:=\widetilde{\nabla}^{2}F(\x^{a}(s))\Big(\x(s)-\x(s-1)\Big)$ where $\widetilde{\nabla}^{2}F$ is an unbiased estimator of $\nabla^{2}F$. Following this idea, we proceed to demonstrate how to estimate the second-order derivative  of the Multinoulli Extension, i.e., 

\begin{theorem}[Proof provided in \cref{append:proof4}]\label{thm4}
	For a set function $f:2^{\V}\rightarrow\R_{+}$, the second-order derivative of its Multinoulli Extension $F$ at any point $(\p_{1},\dots,\p_{K})\in\prod_{k=1}^{K}\Delta_{n_{k}}$ can be  written as follows: 
	
\textbf{1):} If $k_{1}\neq k_{2}\in[K]$, for any $m_{1}\in[n_{k_1}]$ and $m_{2}\in[n_{k_2}]$,
\begin{equation*}
\frac{\partial^{2}F}{\partial p_{k_{1}}^{m_{1}}\partial p_{k_{2}}^{m_{2}}}=B_{k_{1}}B_{k_{2}}\E_{e_{\hat{k}}^{\hat{b}}}\Big(f\big(v_{k_{1}}^{m_{1}}|S\cup\{v_{k_{2}}^{m_{2}}\}\big)-f\big(v_{k_{1}}^{m_{1}}|S\big)\Big),
\end{equation*} 
where $S=\cup_{\hat{k}=1}^{K}\cup_{\hat{b}=1}^{B_{k}}\{e_{\hat{k}}^{\hat{b}}\}\setminus\{e_{k_{1}}^{1},e_{k_{2}}^{1}\}$ and each  $e_{\hat{k}}^{\hat{b}}$ is drawn from the multinoulli distribution Multi($\p_{\hat{k}}$); 

\textbf{2):} As for $k_{1}=k_{2}=k\in[K]$, if $d_{k}=1$, for any $m_{1},m_{2}\in[n_{k}]$, we have $\frac{\partial^{2}F}{\partial p_{k}^{m_{1}}\partial p_{k}^{m_{2}}}=0$; Moreover, when $d_{k}\ge2$, 
\begin{equation*}
	\frac{\partial^{2}F}{\partial p_{k}^{m_{1}}\partial p_{k}^{m_{2}}}=(B_{k}^{2}-B_{k})\E_{e_{\hat{k}}^{\hat{b}}}\Big(f\big(v_{k}^{m_{1}}|S\cup\{v_{k}^{m_{2}}\}\big)-f\big(v_{k}^{m_{1}}|S\big)\Big), 
\end{equation*} where $S=\cup_{\hat{k}=1}^{K}\cup_{\hat{b}=1}^{B_{k}}\{e_{\hat{k}}^{\hat{b}}\}\setminus\{e_{k}^{1},e_{k}^{2}\}$ and each  $e_{\hat{k}}^{\hat{b}}$ is independently drawn from the multinoulli distribution Multi($\p_{\hat{k}}$). 
\end{theorem}
\begin{remark}~\label{remark:estimate_2_order}
Theorem~\ref{thm4}  provides a detailed characterization of the second-order derivative of our proposed Multinoulli Extension $F$, which implies that we can estimate the Hessian of $F$  by sampling a sequence of random elements. Specifically, when each $e_{\hat{k}}^{\hat{b}}$ is independently drawn from the multinoulli distribution Multi($\p_{\hat{k}}$) for any $\hat{k}\in[K]$ and $\hat{b}\in[B_{\hat{k}}] $, we can estimate $\frac{\partial^{2}F}{\partial p_{k_{1}}^{m_{1}}\partial p_{k_{2}}^{m_{2}}}$ as:
 If $k_{1}\neq k_{2}\in[K]$,  
\begin{equation*}
\widehat{\frac{\partial^{2}F}{\partial p_{k_{1}}^{m_{1}}\partial p_{k_{2}}^{m_{2}}}}:=B_{k_{1}}B_{k_{2}}\Big(f\big(v_{k_{1}}^{m_{1}}|S\cup\{v_{k_{2}}^{m_{2}}\}\big)-f\big(v_{k_{1}}^{m_{1}}|S\big)\Big),
\end{equation*} where $S=\cup_{\hat{k}=1}^{K}\cup_{\hat{b}=1}^{B_{k}}\{e_{\hat{k}}^{\hat{b}}\}\setminus\{e_{k_{1}}^{1},e_{k_{2}}^{1}\}$; As for $k_{1}=k_{2}=k\in[K]$ and $d_{k}\ge2$,  
\begin{equation*}
\widehat{\frac{\partial^{2}F}{\partial p_{k}^{m_{1}}\partial p_{k}^{m_{2}}}}:=(B_{k}^{2}-B_{k})\Big(f\big(v_{k}^{m_{1}}|S\cup\{v_{k}^{m_{2}}\}\big)-f\big(v_{k}^{m_{1}}|S\big)\Big),
\end{equation*} where $S=\cup_{\hat{k}=1}^{K}\cup_{\hat{b}=1}^{B_{k}}\{e_{\hat{k}}^{\hat{b}}\}\setminus\{e_{k}^{1},e_{k}^{2}\}$. 
\end{remark}
Incorporating this second-order approximation and the idea of differential estimator into the framework of CG algorithm, we finally can get a stochastic Frank-Wolfe method for maximizing our introduced Multinoulli Extension, as detailed in Algorithm~\ref{alg:scg_mutli}. Similarly, based on Theorem~\ref{thm1} and Theorem~\ref{thm2}, we also can verify that
\begin{theorem}[Proof provided in \cref{append:proof5}]\label{thm5}When the set function $f:2^{\V}\rightarrow\R_{+}$ is monotone and $\alpha$-weakly DR-submodular, if we set the batch size $L=\mathcal{O}(T)$, the subset $S$ output by Algorithm~\ref{alg:scg_mutli} satisfies:
	\begin{equation*}
		\E\big(f(S)\big)\ge\Big(1-e^{-\alpha}\Big)f(S^{*})-\mathcal{O}(\frac{1}{T}),
	\end{equation*} where $S^{*}$ is the optimal solution of problem~\eqref{equ_problem}. Similarly, if the set function $f:2^{\V}\rightarrow\R_{+}$ is $(\gamma,\beta)$-weakly monotone submodular and $L=\mathcal{O}(L=\mathcal{O}(T))$, the returned  subset $S$ of Algorithm~\ref{alg:scg_mutli} satisfies:
	\begin{equation*}
		\E\big(f(S)\big)\ge\Big(\frac{\gamma^{2}(1-e^{-(\beta(1-\gamma)+\gamma^2)})}{\beta(1-\gamma)+\gamma^2}\Big)f(S^{*})-\mathcal{O}(\frac{1}{T}).
	\end{equation*} 
\end{theorem}
\begin{remark}
	Theorem~\ref{thm5} implies that, if the set function $f$  is monotone and $\alpha$-weakly DR-submodular,  after $\mathcal{O}(1/\epsilon)$ iterations and $\mathcal{O}(1/\epsilon^{2})$ evaluations, the returned subset of our proposed Algorithm~\ref{thm2} can attain the $(1-e^{-\alpha})OPT-\epsilon$. Moreover, when $f$ is $(\gamma,\beta)$-weakly monotone  submodular, Algorithm~\ref{thm2} also can achieve $\Big(\frac{\gamma^{2}(1-e^{-(\beta(1-\gamma)+\gamma^2)})}{\beta(1-\gamma)+\gamma^2}\Big)OPT-\epsilon$ after $\mathcal{O}(\frac{1}{\epsilon})$ iterations and $\mathcal{O}(1/\epsilon^{2})$ queries. 
\end{remark}
Compared to the local search methods~\citep{thiery2022two,JOGO-Lu}, our proposed Algorithm~\ref{alg:scg_mutli} not only eliminates the need for prior knowledge of parameters $\alpha$, $\gamma$, and $\beta$, but can achieve the same worst-case approximation guarantees with fewer $\mathcal{O}(\frac{1}{\epsilon^2})$ queries to the set function $f$.








==> authors.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Photos/zhangqx.jpg}}]{Qixin Zhang }
received his B.S. degree from the University of Science and Technology of China (USTC) in 2018. He subsequently earned his Ph.D. degree in the College of Computing at City University of Hong Kong in 2024. Currently, he is a Research Fellow at Nanyang Technological University, Singapore. His research interests include submodular optimization, subset selection, online learning and network pruning. He has published over 15 papers in top-tier venues such as ICML, NeurIPS and ICLR, etc.
\end{IEEEbiography}

\begin{IEEEbiography}
[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Photos/Wei_Huang.jpg}}]{Wei Huang} is a Research Scientist in the Deep Learning Theory Team at RIKEN AIP, Tokyo. He obtained his Ph.D. in Computer Science from the University of Technology Sydney, and holds a Master’s degree in Statistical Physics from the University of Science and Technology of China. Dr. Huang focuses on exploring the theoretical foundations of interpretability and transparency in deep learning’s expressivity, optimization and generalization, as well as on developing new algorithms, models, and methodologies that enhance the interpretability and improve their performance. His contributions to the field are documented in publications such as NeurIPS, ICLR, and ICML et al. He has served as area chair for NeurIPS, ICLR, and AISTATS, and received the CPAL 2025 and KAUST 2025 Rising Star Awards.
\end{IEEEbiography}\vspace{-1.0em}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Photos/yansun.jpg}}]{Yan~Sun} received his B.Eng. degree in electronic and information engineering from University of Science and Technology of China (USTC) in 2018. He is currently a Ph.D. candidate at the University of Sydney (USYD). His current research area includes large-scale training, federated learning, machine learning, and learning theory.
\end{IEEEbiography}\vspace{-1.0em}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{Photos/Yao SHU.jpg}}]{Yao Shu}received the B.Eng. degree from Huazhong University of Science and Technology, China, in 2017, and the Ph.D. degree from the National University of Singapore, Singapore, in 2022. He is currently a Tenure-Track Assistant Professor in the Artificial Intelligence Thrust, The Hong Kong University of Science and Technology (Guangzhou), China. His research interests include deep learning theory and optimization algorithms.
\end{IEEEbiography}\vspace{-1.0em}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{./Photos/Yi_Yu.jpg}}]
    {Yi Yu} 
    received the B.Eng. degree from the Department of Automation, Tsinghua University, China, the M.S. degree from the Department of Electrical and Computer Engineering, University of California San Diego, United States, and the Ph.D. degree from Nanyang Technological University (NTU), Singapore in 2019, 2021 and 2025, respectively. He is currently a Postdoctoral Research Fellow at Nanyang Technological University, Singapore.
    %
    His research interests include adversarial robustness, trustworthy ML, and AI security.  
    % He serves as a regular reviewer member for IEEE TPAMI, IEEE TIP, IEEE TMM, Neurips, ICML and CVPR.
\end{IEEEbiography}\vspace{-1.0em}


\begin{IEEEbiography}
[{\includegraphics[height=1.25in,clip,keepaspectratio]{Photos/tao_dc.jpg}}]{Dacheng Tao}(F’15) is currently a Distinguished University Professor in the College of Computing \& Data Science at Nanyang Technological University. He mainly applies statistics and mathematics to artificial intelligence and data science, and his research is detailed in one monograph and over 200 publications in prestigious journals and proceedings at leading conferences, with best paper awards, best student paper awards, and test-of-time awards. His publications have been cited over 173K times and he has an h-index 200+ in Google Scholar. He received the 2015 and 2020 Australian Eureka Prize, the 2018 IEEE ICDM Research Contributions Award, and the 2021 IEEE Computer Society McCluskey Technical Achievement Award. He is a Fellow of the Australian Academy of Science, AAAS, ACM and IEEE.
\end{IEEEbiography}
